The Linked Data Benchmark Council (LDBC): Driving competition and collaboration in the graph data management space

Graph data management is instrumental for several use cases such as recommendation, root cause analysis, financial fraud detection, and enterprise knowledge representation. Efficiently supporting these use cases yields a number of unique requirements, including the need for a concise query language and graph-aware query optimization techniques. The goal of the Linked Data Benchmark Council (LDBC) is to design a set of standard benchmarks that capture representative categories of graph data management problems, making the performance of systems comparable and facilitating competition among vendors. LDBC also conducts research on graph schemas and graph query languages. This paper introduces the LDBC organization and its work over the last decade.

==> acknowledgements.tex <==
\section*{Acknowledgements}


We would like to thank all our past and present members for their contributions in our working groups and task forces.


==> bottom.tex <==

\setcounter{tocdepth}{3}
\tableofcontents

\section*{Important dates}

\begin{itemize}
    \item Abstract due: June 14th, 2023
    \item Papers due: June 21st, 2023
    \item Notification of acceptance: June 28th, 2023
    \item Conference day: August 28st, 2023
\end{itemize}


==> community.tex <==
\section{Community}
\label{sec:community}


==> delete-operations.tex <==
\section{Temporal Graph Generation}
\label{sec:temporal-graph-generation}

\input{figures/fig-serialization-conds}

\input{figures/fig-comments}

\subsection{Lifespan Management}
\label{sec:lifespan-management}

\subsection{Insert Operations}
\label{sec:insert-operations}

\subsection{Delete Operations}
\label{sec:delete-operations}

\subsection{Serialization Conditions}
\label{sec:serialization-conditions}

\autoref{fig:serialization-conds}


explicit vs. implicit deletes

distributions

\input{figures/fig-data-set}


==> evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

\paragraph{Disclaimer.}
The experiments presented here are {\bf not} LDBC Benchmark Results, as they were not {\em audited} and do not include price-adjusted scores.
Their purpose is solely to demonstrate the expected performance impact of introducing delete operations to the upcoming SNB Interactive workload.

\subsection{Benchmark Enviroment}
\label{sec:benchmark-environment}

The experiments were run in AWS EC2 on an \texttt{r5d.16xlarge} instance (64 Intel Xeon Platinum 8259CL vCPU cores at 2.50~GHz, 512~GiB RAM, 4~NVMe SSDs in RAID-0 configuration) with Fedora Linux~34.
The SUTs were run in a containerized environment using Docker~20.10.

\subsection{Analysis of the Results}
\label{sec:analysis-of-the-results}




==> figure-delete-operations.tex <==
\begin{figure}[htb]
    \Description[]
    \centering
    \includegraphics[scale=\yedscale]{figures/schema-compact}
    \caption{
      Entities in the social network schema.
      Many-to-many edges are highlighted with thick lines.
      The \Knows edges are undirected, while the rest of the edges are directed.
    }
    \label{fig:schema}

    \includegraphics[scale=\yedscale]{figures/example-graph.pdf}
    \caption{Deleting a \Forum in an example graph.
    Dashed nodes and edges are deleted due to the \text{Forum}'s deletion.
    }
    \label{fig:example-delete}
\end{figure}


==> related-work.tex <==
\section{Related Work}
\label{sec:related-work}

\subsection*{Traditional OLTP Benchmarks}

Traditional transaction processing benchmarks contain write-heavy transactions and
non-trivial relations. For example, in TPC-C~\cite{tpcc} only 8\% transactions are
read-only. In these benchmarks transactions containing delete operations are
under-represented, and when they do feature are simple. To illustrate consider
BenchBase~\cite{DBLP:journals/pvldb/DifallahPCC13}, an open-source DBMS
benchmarking platform, which contains six popular OLTP  benchmarks. Only
TPCC (\texttt{Delivery}), SEATS (\texttt{DeleteReservation}), and TATP
(\texttt{DeleteCallForwarding}) contained a transaction with a delete operation.
Compared to SNB Interactive, these transactions are simple at most deleting data from a
single table, whereas \texttt{DeletePerson} accesses ?

\subsection*{Microbenchmarks}
\label{sec:microbenchmarks}

\begin{itemize}
\item Graph Microbench.~\cite{DBLP:journals/pvldb/LissandriniBV18}.
\item YCSB
\end{itemize}

Delete transactions: YCSB (DeleteRecord)

\subsection*{Transactional Graph Benchmarks}

\begin{itemize}
\item LinkBench~\cite{DBLP:conf/sigmod/ArmstrongPBC13}.
\item TAOBench~\cite{TAOBench}.
\item LDBC SNB Interactive~\cite{DBLP:conf/sigmod/ErlingALCGPPB15}.
\item BG~\cite{DBLP:journals/fgcs/AlabdulkarimBG18},
\item Epinions (BenchBase)
\item Twitter (BenchBase)
\item Wikipedia (BenchBase)
\end{itemize}

Delete transactions: wikipedia (RemoveWatchList)
Use large-scale data sets, only contains simple reads (lookups) and simple updates.

\subsection*{Analytical Benchmarks}

\begin{itemize}
\item \tpcH~\cite{tpch},
\item \tpcDS~\cite{tpcds,DBLP:conf/cloud/PoessRJ17},
\item LDBC SNB BI~\cite{DBLP:conf/grades/SzarnyasPAMPKEB18,DBLP:journals/corr/abs-2001-02299}
\item BSMA~\cite{DBLP:journals/pvldb/XiaLYMQ14}
\item Train Benchmark~\cite{DBLP:journals/sosym/SzarnyasIRV18},
\end{itemize}

\subsection*{RDF/Semantic Web}

\begin{itemize}
\item LUBM~\cite{DBLP:journals/ws/GuoPH05}.
\item BSBM~\cite{DBLP:journals/ijswis/BizerS09}.
\item SP\textsuperscript{2}Bench~\cite{DBLP:books/sp/virgilio09/SchmidtHMPL09}.
\item WatDiv~\cite{DBLP:conf/semweb/AlucHOD14}
\end{itemize}


==> tab-graphalytics.tex <==
\begin{table}[htb]
    \centering
    \setlength\tabcolsep{3.0pt}
    \scriptsize
    \begin{tabular}{@{}l|r|rrrrrr|r@{}}
        \toprule
        \theadbar{System}        & \theadbar{Load time} & \thead{BFS} & \thead{CDLP} & \thead{LCC} & \thead{PR} & \thead{SSSP} & \theadbar{WCC} & \thead{Price}         \\
        \midrule
        results TBA \\
        \bottomrule
    \end{tabular}
    \caption{The global leaderboard of the LDBC Graphalytics 2023 competition. Load times are reported in seconds. TODO: ranking should be displayed.}
    \label{tab:graphalytics-leaderboard}
\end{table}

